GL-CLeF: A Global-Local Contrastive Learning Framework for Cross-lingual Spoken Language Understanding

Due to high data demands of current methods, attention to zero-shot cross-lingual spoken language understanding (SLU) has grown, as such approaches greatly reduce human annotation effort. However, existing models solely rely on shared parameters, which can only perform implicit alignment across languages. We present Global--Local Contrastive Learning Framework (GL-CLeF) to address this shortcoming. Specifically, we employ contrastive learning, leveraging bilingual dictionaries to construct multilingual views of the same utterance, then encourage their representations to be more similar than negative example pairs, which achieves to explicitly aligned representations of similar sentences across languages. In addition, a key step in GL-CLeF is a proposed Local and Global component, which achieves a fine-grained cross-lingual transfer (i.e., sentence-level Local intent transfer, token-level Local slot transfer, and semantic-level Global transfer across intent and slot). Experiments on MultiATIS++ show that GL-CLeF achieves the best performance and successfully pulls representations of similar sentences across languages closer.

==> Approach.tex <==


The detailed statistics of EToDR are summarized in Table~\ref{table:statistic}.
%Table~\ref{table:statistic} lists the statistic comparison between the original SMD ddataset and EToDR dataset.
Compared with the original SMD dataset, EToDR annotates \textit{supporting facts} information and fix the weaknesses mentioned in Section~\ref{Introduction}, which allows direct evaluation of reasoning over KB. In total, we hire 15 experts to take part in the annotation process, which lasts six months.

%The {EToDR} data collection procedure includes three steps: (1) \textit{Empty KB Dialogues Removal}, (2) \textit{Unanswerable Dialogues Creation} and (3) \textit{Support Facts Annotation}.
\begin{table}[t] 
	\centering
	\begin{adjustbox}{width=0.35\textwidth}
		\begin{tabular}{c|c}
			& {EToDR} \\
			\hline
			\# Training Dialogues & 2,011\\
			\# Validation Dialogues & 242\\
			\# Test Dialogues & 256\\
			Vocabulary Size & 1,671 \\
			\# Utterances & 16,362 \\
			\# Unanswerable Dialogues & 1,287 \\
			\# Support Facts & 10,307 \\
			\# Avg. Turns per Dialogue & 3.26 \\
			\# Avg. Words per Utterance & 7.88 \\
			\hline
		\end{tabular}
	\end{adjustbox}
	\caption{Data statistics of EToDR.}
	\label{table:statistic}
	% \vspace{-10pt}
\end{table}
%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.187]{./pictures/template.pdf}
%	\caption{
%		A snippet of templates for each domain. The KB entity is removed and replaced with the delexicalized slot tag, which is shown in bold font. The complete templates can be found in the Appendix C.
%	}
%	\label{fig:templates}
%\end{figure}
\subsection{Empty KB Dialogues Removed}
Empty KB dialogues have dialogue utterances without corresponding KB.
We find that 17.9\% of dialogues in SMD have empty KB, and a model trained on the dialogues with empty KB only needs to copy entities from dialog history.
Therefore, we remove such dialogues with empty KB in order to encourage a model to rely on the corresponding KB for retrieving the relevant entities. 
%Thus, in \textit{EToDR}, all dialogues have their corresponding KB.


%\begin{figure}[t]
%	\centering
%	\begin{tabular}[t]{ p{2.7cm} | p{4cm} }
%		%\toprule
%		\textbf{Domain} & \textbf{Template} \\\hline
%		\textit{Navigate} & Your ride is booked and the cab is on its way. \\
%	& Have a safe ride!\\ \hline
%		\textit{request(dest)} & Where are you riding to?\\
%		\textit{request(shared)} & Are you comfortable sharing the ride?\\ \hline
%		\textit{confirm(dest=}\$x\textit{)} & You are going to \$x. \\
%		\textit{inform(fare=}\$x\textit{)} & Your ride costs \$x dollars. \\
%		\textit{inform(seats=}\$x\textit{)} & The cab is for \$x riders.
%	\end{tabular}
%	\caption{Example templates for each domain. The KB entity is removed and replaced with the delexicalized slot tag.}
%	\label{fig:templates}
%\end{figure}


\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{./pictures/Figure4-support-fact-annotation.pdf}
	\caption{ Support fact annotation process.
	}
	\label{fig:support}
\end{figure*}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{./pictures/Figure3-case-for-unanswerable-question.pdf}
	\caption{ Unanswerable questions insertion process.
%		 (a) The original dialogues. (b) The created unanswerable question-answer pairs. (c) New dialogues with answerable query.
	}
	\label{fig:case-for-insertion}
\end{figure}
\subsection{Unanswerable Dialogues Creation}
%Instead of SMD that mainly query the entity that exists in dialog history or KB, which 
%We argue that the existing SMD's focus on queries for which the corresponding knowledge entity is guaranteed to exist in dialog history most of the time, which causes that model only need to copy and memorize the knowledge entity from dialog history, instead of reasoning over KB to query the relevant entity.
Inspired by~\citet{rajpurkar-etal-2018-know}, we construct unanswerable dialogues to improve the difficulty of the dataset.
%hoping to evaluate whether a model is able to successfully understand KB rather than simply “\texttt{copy}” entity span from dialog history.
%The motivation behind is that 
If a model can respond to the unanswerable dialogues, which means that the model perform reasoning over KB to successfully understand that the corresponding KB can not support the current dialog.
%More specifically, the creation process has two steps: 
Unanswerable dialogues are made in two steps:
\textit{unanswerable questions creation} and \textit{inserted into original dialogues}. 

% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{./pictures/Figure5-typo-comparison.pdf}
% 	\caption{ Examples of annotation errors between SMD and \textsc{EtoDR}.
% 	}
% 	\label{fig:typos_comparison}
% \end{figure*}

\paragraph{Step 1 Unanswerable Questions Creation:}
%\qlbcomment{maybe, we can use algorithm format to describe the detail of process.}
We first adopt delexicalization, where all knowledge entities are replaced by their corresponding slot (such value:\texttt{3pm}-$>$slot:\texttt{time}).
% to create the unanswerable question templates. 
%
%We use a simple heuristic rule to create some unanswerable question templates in each domain, which are shown in Figure~\ref{fig:templates}. 
% and create various of questions. The step is shown in Figure?. 
To ensure diversity and richness, we construct about 30 types of templates for each domain.\footnote{The detailed templates can be found in the Appendix C.}
%, which are shown in  Figure~\ref{fig:templates}.
% and the template cannot include the specific slot-value but use the slot name to replace the value.
Next, for generating unanswerable questions, we sample specific entities from the whole KB to replace the generated slot and ensure that the sampled KB entity is beyond the scope of the corresponding KB.
By this means, the created questions cannot be answered with the corresponding KB.
For the response generation for the unanswerable query, we generate a similar response (\textit{Sorry, I can't find the entity type in the corresponding KB.}).
Finally, the unanswerable question-answer pairs are created.
%, which can avoid to fuse the model.
\paragraph{Step 2 Insertion into Original Dialogues:}
After obtaining unanswerable question-answer pairs, we consider how to insert them into the original dialogues.
Since utterances in dialogue should keep coherence and logic-consistence, 
%we cannot only randomly insert the generated unanswerable question-response pair into the original dialogues. As a solution, 
we insert unanswerable questions at the beginning of the original dialogue, which not only increases the difficulty of the original data but also ensures the logical consistency of the dialogue.
In addition, we ask experts to check whether the constructed dialogues are fluent or not and remove these incoherent dialogues.
An example is shown in Figure~\ref{fig:case-for-insertion}.
%\qlbcomment{可以举一个例子说明！}
In this way, we insert unanswerable dialogue pairs into 70\% of original conversations.


\subsection{Supporting Fact Annotation}
One core contribution in our paper is that instead of simply giving an appropriate response, we also require a model to identify the corresponding \textit{supporting facts} that the knowledge entity is actually derived from. 
This operation can help guide the model to perform meaningful and explainable reasoning.
%In the paper, we hope our dialog systems not only to give an appropriate response but also to identify \textit{supporting KB row}.
%Hence, we need to annotate the \textit{supporting KB row} for each utterance in a dialog.
%To equip the original SMD with support facts for each response, 
We choose a coarse-to-fine method to conduct annotation.
It includes two steps (\textit{Candidate Support facts Selection} and \textit{Accurate Support Facts Location}), as illustrated in Figure~\ref{fig:support}.
\paragraph{Step 1 Candidate Selection:}
For the coarse step, we adopt a simple string matching method to obtain the candidate KB rows.
%\footnote{It is worth noting that we cannot guarantee that all candidate rows are picked out by simple string matching (recall 69\%), and thus annotators further re-check to prevent missing recall the supporting fact.}
%To reduce the efforts of human annotation, we first adopt the string matching method to obtain the candidate KB rows.
Given each entity in response, we scan the whole KB and select the KB row which includes the entity.
Take the dialogue in Figure~\ref{fig:support} for example,
the entity “\texttt{father}” matches 4 rows in KB (the first, second, fifth, and seventh rows), and the matched KB rows are selected.
Similarly, given the entity “\texttt{jeff}”, the matched sixth KB row is selected.
%a
%
% six KB rows that include are selected
%Taking the dialogue in Figure for an example, the similarity of the 4 th row equals to \texttt{4} with :“\texttt{200 Alester Ave}”, “\texttt{gas station}”, “\texttt{Valero}”, and “\texttt{road block nearby}” matching the dialogue context; and the similarity of the 7 th row equals to 1 with only “road block nearby” matching.

\paragraph{Step 2 Supporting Fact Labeling:}
Since there may be multiple identical entities in the same KB, simple string matching can cause inconsistent annotation.
As shown in Figure~\ref{fig:support}(b), six KB rows are selected by Step 1.
However, except for the first and the sixth rows, the other supporting facts have a conflict with the entity “\texttt{optometrist\_apointment}”.
To address this issue, 
%Since the simply string matching may cause the incorrect KB row collection, 
we ask experts to manually fix the error.
For each annotated support fact, three experts check the automatic annotation results.
If there is an error in \textit{support fact} and he can write the correct annotation.
Finally, he/she must ask for another two experts to check his/her re-annotated result until three experts have a consistent agreement.
The corrected support facts annotation is illustrated in Figure~\ref{fig:support}(c).


%\subsection{Dataset Statistics}

%\begin{table}[t] 
%	\centering
%	\begin{adjustbox}{width=0.35\textwidth}
%		\begin{tabular}{c|c}
%			& EToDR \\
%			\hline
%			\# Training Dialogues & 8,860\\
%			\# Validation Dialogues & 4.73\\
%			\# Test Dialogues & 19.57\\
%			Vocabulary Size & 8,809 \\
%			\# Utterances & 8,943 \\
%			\# Unanswerable Dialogues & 11,343 \\
%			\# Support Facts & 6,371 \\
%			\# Avg. Turns per Dialogue & 11,323 \\
%			\# Avg. Words per Utterance & 4\\
%			\hline
%		\end{tabular}
%	\end{adjustbox}
%	\caption{Data statistics of EToDR.}
%	\label{table:statistic}
%	\vspace{-10pt}
%\end{table}



\subsection{Quality Control}
%
%Annotators in Step 2 are all NLP-major master students in Chinese, who are familiar with dialog topic and fluent in English (pass the CET-6\footnote{The highest level test for NLP-majors student in China.}). Annotators are required to draft annotate 170 instances repeatedly until their labeling is sufﬁciently accurate to provide useful annotation. Because not all conversations are adapted to construct a reasoning-based response problem, the annotator has the right to skip the conversation. We employ ﬁve annotators to construct the response, and two quality inspectors to check it. We discard the instance when inspectors doubt the uniqueness or correctness of the answer.
%To control the quality of the annotated dataset, we introduce different verification methods:
%
%First, in the annotation process, we review 200 randomly sampled tuples every 10,000 annotations. We assign a ``gold'' label to each tuple and then decided whether the whole annotation batch should be accepted or re-annotated according to the disagreement rate. With tolerance to the different understandings of the dialogue response, we set an empirical acceptance threshold of disagreement rate to 10\%. For the majority of annotated batches, the disagreement rate varies from 3\% to 7\%. 
%
%The second verification is conducted by paid annotators. Each consistency label is verified by two annotators. The tuples with a low inter-annotator agreement in their labels are directly discarded from the final dataset. Finally, we obtain 118,540 tuples in the KvPI dataset.

%\textit{support fact} annotated dataset, 
To control the quality of the annotated dataset, we make the following efforts: (1) \textbf{Verification}: We randomly sampled 2,000 question-response pairs from the final annotated dataset and ask two new annotators to annotate the corresponding \textit{supporting facts}, as in the completed annotation process. Following~\citet{bowman-etal-2015-large}, we calculated the Fleiss' Kappa among the previous labels and two new labels and obtained a kappa of 0.867, which indicates {\it an almost perfect agreement}~\citep{landis1977measurement};
(2) \textbf{Additional Annotations}:  SMD was collected using a Wizard-of-OZ \cite{kelley1984iterative} setup.
	It has been shown that the values annotated by the Wizard were not guaranteed to be consistent with the underlying database ontology \cite{eric2019multiwoz}.
	We re-annotate EToDR to fix the mistakes existed in the original SMD.
%	 (1) {\textit{Missing Entities}}. These refer to knowledge entities that miss some subword compared with the gold annotation. 
%	% Row 1 of Figure~\ref{fig:typos_comparison} shows this case where entity \textit{Stanford Oval} misses the subword \textit{Parking};
%	(2){ \textit{Fact Contradiction}}. The annotation entity has a conflict with the gold annotation. 
%	% In row 2 of Figure~\ref{fig:typos_comparison} shows such a case where \textit{hot} has a conflict with \textit{hail};
%	(3) {\textit{Typos}}. The annotated entity is a typo. 
%	% Row 3 of Figure~\ref{fig:typos_comparison} exhibits such a case with \textit{Atheron};
%	(4) {\textit{Normalization Errors}}.  These refer to annotations that are not normalized between the utterance and KB.  
	More detailed explanations can be found at Appendix B.
%We randomly sampled 2,000 question-response pairs from the final annotated dataset and ask two new annotators to annotate the corresponding \textit{supporting facts}, as in the completed annotation process. Following~\citet{bowman-etal-2015-large}, we calculated the Fleiss' Kappa among the previous labels and two new labels and obtained a kappa of 0.867, which indicates {\it an almost perfect agreement}~\citep{landis1977measurement}. 
%%This result shows that the completed annotation is of reliable quality.


% \subsection{Additional Corrections to SMD}
% SMD was collected using a Wizard-of-OZ \cite{kelley1984iterative} setup.
% It has been shown that the values annotated by the Wizard were not guaranteed to be consistent with the underlying database ontology \cite{eric2019multiwoz}.
% We fix the following mistakes made by the crowd-workers with human efforts: (1) \textbf{\textit{Missing Entities}}. These refer to knowledge entities that miss some subword compared with the gold annotation. 
%% Row 1 of Figure~\ref{fig:typos_comparison} shows this case where entity \textit{Stanford Oval} misses the subword \textit{Parking};
% (2)\textbf{ \textit{Fact Contradiction}}. The annotation entity has a conflict with the gold annotation. 
%% In row 2 of Figure~\ref{fig:typos_comparison} shows such a case where \textit{hot} has a conflict with \textit{hail};
% (3) \textbf{\textit{Typos}}. The annotated entity is a typo. 
%% Row 3 of Figure~\ref{fig:typos_comparison} exhibits such a case with \textit{Atheron};
% (4) \textbf{\textit{Normalization Errors}}.  These refer to annotations that are not normalized between the utterance and KB. 
%% 
%% Row 4 of Figure~\ref{fig:typos_comparison} shows the case that \textit{one miles} should be annotated as \textit{1 miles}.
%More detailed explanations can be found at Appendix B.
%%\begin{itemize}
%%	\item \textit{Missing Entities}. These refer to knowledge entities that miss some subword compared with the gold annotation. Row 1 of Figure~\ref{fig:typos_comparison} shows this case where entity \textit{Stanford Oval} misses the subword \textit{Parking}. 
%%	\item \textit{Fact Contradiction}. The annotation entity has a conflict with the gold annotation. In row 2 of Figure~\ref{fig:typos_comparison} shows such a case where \textit{hot} has a conflict with \textit{hail}.
%%	\item \textit{Typos}. The annotated entity is a typo. Row 3 of Figure~\ref{fig:typos_comparison} exhibits such a case with \textit{Atheron}.
%%	\item \textit{Normalization Errors}.  These refer to annotations that are not normalized between the utterance and KB. Row 4 of Figure~\ref{fig:typos_comparison} shows the case that \textit{one miles} should be annotated as \textit{1 miles}.
%%%	The annotation problem affects the automatic evaluation. 
%%	
%%\end{itemize}

==> plot.tex <==
\usepackage{tikz}
\usepackage{pgfplots}


\pgfplotstableread[row sep=\\,col sep=&]{
    Scale & wtq & sqa & tabfact & wiki \\
    $0.1$   & 48.6 & 65.3 & 82.8 & 88.1 \\
    $0.5$   & 54.2 & 68.1 & 83.6  & 88.8\\
    $1.0$   & 56.1 & 70.2 & 83.8  & 89.2 \\
    $5.0$  & 57.0 & 70.3  & 84.6  & 89.1 \\
    }\mydata

\pgfplotsset{every axis/.append style={
                    label style={font=\large},
                    tick label style={font=\large} 
                    }}
\begin{figure}[t!]
    \centering
    \begin{tikzpicture}[scale=0.7]
        \begin{axis}[
                ybar=5pt,
                bar width=.33cm,
                enlarge x limits=0.2,
                width=1.4\textwidth,
                height=.7\textwidth,
                legend style={at={(0.5,1.20)},
                anchor=north,legend columns=-1},
                symbolic x coords={$0.1$, $0.5$, $1.0$, $5.0$},
                xtick=data,
                nodes near coords,
                every node near coord/.append style={font=\small},
                nodes near coords align={vertical},
                ymin=40,ymax=100,
                ylabel={Task Performance (\%)},
                xlabel={Amount of Pretraining Corpus (Millions)}
            ]
            \addplot table[x=Scale,y=wtq]{\mydata};
            \addplot table[x=Scale,y=sqa]{\mydata};
            \addplot table[x=Scale,y=tabfact]{\mydata};
            \addplot table[x=Scale,y=wiki]{\mydata};
            \legend{\wtq, \sqa, \tabfact, \wikisql}
        \end{axis}
    \end{tikzpicture}
    \caption{The illustration of downstream tasks performance with different scales of pre-training corpus. Scaling up the pre-training corpus of \ours generally brings positive effects across datasets.}
\end{figure}
